TIF: Learning Temporal Invariance in Android Malware Detectors

Learning-based Android malware detectors degrade over time due to natural distribution drift caused by malware variants and new families. This paper systematically investigates the challenges classifiers trained with empirical risk minimization (ERM) face against such distribution shifts and attributes their shortcomings to their inability to learn \emph{stable} discriminative features. Invariant learning theory offers a promising solution by encouraging models to generate stable representations across environments that expose the instability of the training set. However, the lack of prior environment labels, the diversity of drift factors, and low-quality representations caused by diverse families make this task challenging. To address these issues, we propose TIF, the first temporal invariant training framework for malware detection, which aims to enhance the ability of detectors to learn stable representations across time. TIF organizes environments based on application observation dates to reveal temporal drift, integrating specialized multi-proxy contrastive learning and invariant gradient alignment to generate and align environments with high-quality, stable representations. TIF can be seamlessly integrated into any learning-based detector. Experiments on a decade-long dataset show that TIF excels, particularly in early deployment stages, addressing real-world needs and outperforming state-of-the-art methods.

==> Table/RQ2.tex <==
\begin{table}[!t]
\small
\caption{F1 of classifiers in non-drift, closed-world drift and open-world test scenarios after adding different schemes in different feature spaces. AG, GR and TS represent the three baselines, APIGraph~\cite{apigraph}, GuideRetraining~\cite{guide_retraining} and T-stability~\cite{svm_ce} respectively}
\centering
% \label{tab: rq2}
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {c=2}{},
  cell{2}{1} = {r=6}{},
  cell{8}{1} = {r=4}{},
  cell{12}{1} = {r=4}{},
  vline{2,4-5} = {1}{},
  vline{2-5} = {1-7,8-11,12-15}{},
  hline{1-2,8,12,16} = {-}{},
}
Method     &      & I.I.D & {Close\\World} & {Open\\World} \\
{Drebin\\ \cite{Arpdrebin,Grossedeepdrebin}} & w/o  & 0.982 &  0.675 & 0.622           \\
           & TS   & 0.980  & 0.672 &   0.622  \\
           & AG   & 0.991  & 0.713 &  0.611 \\
           & GR   & 0.984 &  0.691  & 0.600\\
           & Ours & 0.992 &  0.792 & 0.648 \\
           & $\Delta$     &     &             &            \\
{Malscan\\~\cite{malscan}}    & w/o  & 0.9433 &    &            \\
           & GR   & 0.9506 &             &            \\
           & Ours & 0.9582 &             &            \\
           & $\Delta$ &     &             &            \\
{BERTDroid\\~\cite{bertroid}}  & w/o  & 0.859 &             &            \\
           & GR   & 0.866 &             &            \\
           & Ours & 0.897 &             &            \\
           & $\Delta$ &     &             &            
\end{tblr}
\end{table}

==> Tex/EthicsConsiderations.tex <==
\section{Ethics Considerations}

This research addresses temporal drift in Android malware detection and introduces a framework named TIF to enhance robustness against such a phenomenon. The apps used in this work are from publicly availablea and anonymized datasets with no personally identifiable information, ensuring compliance with ethical and institutional guidelines. 

All methods are designed solely for academic and security purposes, with no potential for misuse or harm to users. Efforts were made to minimize risks, such as false positives and negatives, and to focus on improving detection stability across evolving malware distributions. The findings are framed strictly to enhance cybersecurity, adhering to principles of beneficence and respect for persons, and contributing positively to public safety and the research community.

==> Tex/OpenScience.tex <==
\section{Open Science}

In alignment with the USENIX Security open science policy, we commit to openly sharing all necessary research artifacts upon the paper’s acceptance and prior to final camera-ready submission. This includes source code, scripts, and metadata about the datasets used in our study. These artifacts will be carefully documented to ensure reproducibility and replicability of our findings. While the datasets themselves are not publicly distributable due to licensing restrictions and the size of samples, comprehensive metadata and usage instructions will be provided to enable the creation of the same dataset. By adhering to these practices, we aim to foster transparency and contribute to the broader adoption of open science principles within the research community.

==> Tex/Rebuttal.tex <==
\vspace{0.5em}
{\large\noindent\textbf{Authors' Response}}
\vspace{0.5em}

We are deeply grateful to the Editor for handling our manuscript and allowing us to revise it. We would also like to thank all Reviewers for their thoughtful and constructive feedback sincerely. Their valuable comments have greatly helped us improve the clarity, completeness, and overall quality of our work.

In response to the reviewers’ feedback, we have carefully revised the manuscript and made the necessary modifications to address all concerns. A detailed, point-by-point response is provided below. The reviewers’ comments are shown in italic, and all significant revisions in the manuscript are highlighted in blue for clarity.

We sincerely appreciate the opportunity to enhance our manuscript and believe that the revisions have substantially strengthened its technical depth and presentation. We hope that the revised version meets the reviewers’ expectations, and we remain happy to provide further clarifications if needed.

\vspace{1.5em}
{\large\noindent\textbf{Response to Reviewer 1}} 

\vspace{0.5em}
\noindent\textbf{Response R1.1 [Main Idea \& Insight]} \textit{The problem to be solved in this paper is clearly explained in the introduction. However, after reading the introduction, the main idea of the proposed approach has not been explicitly explained. What is/are your insight(s) to tackle the problem? Why you think the idea would work?}

We have substantially revised the Introduction (Section~\ref{sec:introduction}) to explicitly articulate the main idea, key insight, and the rationale behind our approach.

1. Our Key Insight: 
We observe that the fundamental limitation of ERM under natural distribution drift is not merely the presence of changing data distributions, but the loss of temporal structure during training. By collapsing samples collected at different time periods into a single static distribution, ERM obscures which correlations are stable over time and which are transient, encouraging shortcut features that are predictive on average but brittle under temporal evolution. Hence, our key insight is that time itself provides weak but consistent supervision: timestamps are not noise, but implicit signals that reveal how malware behavior evolves. Correlations that persist across time are more likely to reflect stable malicious semantics, while those that vary with time tend to encode transient implementation details. Making temporal variation explicit during training enables the learning process to prioritize representations that remain stable despite malware evolution.


2. Why this idea works: 
The effectiveness of \model\ comes from rethinking ERM-based training under natural distribution drift and aligning the training objective with real-world deployment scenarios.

First, TIF changes what information is exposed during training.
Instead of collapsing samples from different time periods into a single static distribution as in ERM, we treat time as an explicit source of environmental variation. This exposes temporally unstable correlations that would otherwise be averaged out, allowing the model to distinguish stable malicious semantics from transient, time-specific artifacts at the representation level.

Second, TIF changes how the model is optimized for generalization.
By partitioning historical data into temporal environments, we instantiate the principle of Invariant Risk Minimization (IRM) by explicitly penalizing representations whose predictive power varies across time. This aligns the optimization process with the deployment scenario, where future samples naturally come from unseen time periods, and encourages the model to rely on temporally invariant correlations rather than spurious historical shortcuts. Importantly, \model\ is not a naive application of invariant learning: the multi-proxy contrastive module is crucial for producing high-quality representations in the presence of heterogeneous malware families, while the environment-specific gradient alignment mitigate known instability issues of IRM, making \model\ tailor to the malware detection setting. These design choices ensure that temporal invariance is not only a theoretical objective, but also a practically learnable property under realistic malware evolution.


% 1) Existence of Invariance: As detailed analysis in the motivation section (Section~\ref{motivation}), we demonstrate that despite rapid changes in implementation, the underlying malicious intent and functional semantics remain relatively stable across time. Such invariance is already implicitly present in historical training data but is overlooked by standard ERM training. 2) Mechanism of Alignment: Our work aligns the training objective with the deployment reality. By partitioning historical data into temporal environments, we simulate the natural distribution drift within the training phase itself. Instead of optimizing for a static average (ERM), \model\ forces the model to solve a harder problem: finding representations that remain stable across these historical time shifts. This explicitly prepares the detector for the testing scenario, ensuring that the learned semantics are not just statistically correlated in the past, but are invariant to the passage of time, thus directly addressing the root cause of degradation.


\vspace{0.5em}
\noindent\textbf{Response R1.2 [Definition of Temporal Invariance]} \textit{what is the definition of ``temporal invariant''? I only knew the meaning of this term until I read the examples in Fig.2. That is too late and also informal.}

We agree that formally defining temporal invariance early in the paper is crucial for understanding our contribution. We have made two revisions to address this:

1. To ensure the concept is understood immediately, we have revised the Introduction (Section~\ref{sec:introduction}, Paragraph 2) to provide an explicit conceptual definition. We clarify that temporal invariance refers to the persistence of malicious intent and functional semantics, even as implementation details (e.g., APIs, obfuscation) evolve over time.

2. To address the concern about informality, we have introduced the explanation of temporal invariance in Section~\ref{sec:Malware Evolution}, including inter- and intra-invariance. We further operationalize this notion in our framework by defining a \textit{Temporally Invariant Feature} as one that simultaneously satisfies Stability (consistency across temporal environments, Eq.~\ref{eq:stability}) and Discriminability (separability between classes, Eq.~\ref{eq:discrim}), with the combined formulation given in Eq.~\ref{eq:invariant}.



\vspace{0.5em}
\noindent\textbf{Response R1.3 [Training Cost]} \textit{How is the cost of using this temporal invariant training framework? Have you reported the time taken to perform training?} 

We have added an Overhead Analysis section (Section~\ref{sec:overhead}) to analyze the training cost of \model\ explicitly. While \model\ exhibits a predictable increase in training computation compared to standard ERM baselines, this is a strategic trade-off to secure performance stability. The additional computation stems from our robust design, specifically temporal environment partitioning, multi-proxy contrastive learning, and two-stage optimization, which is essential for learning drift-resistant representations. Crucially, this upfront training investment yields significant long-term benefits in terms of efficiency. In continual learning scenarios, \model\ demonstrates superior robustness, substantially reducing the frequency of required model updates during deployment. Consequently, although the initial offline training cost is higher, the total lifecycle cost (including retraining and data labeling) is effectively lowered. Furthermore, this design introduces zero overhead at inference time, preserving real-time efficiency. 

\vspace{0.5em}
\noindent\textbf{Response R1.4 [Case Study]} \textit{That is good to see the proposed approach indeed improved the F1-score (and other metrics) over the baselines. Can you give some case studies to showcase the superiority of the proposed approach? Such case studies would allow the readers to understand why you can improve the F1-score and mitigate the problem you aim to solve.}

To provide concrete and interpretable evidence explaining why our method improves F1-score and robustness under temporal drift, we have added a dedicated Case Study in Section~\ref{sec:case study}. Specifically, we analyze the top-10 important features in the interpretable Drebin feature space, comparing \model\ with the ERM-based baseline DeepDrebin~\cite{Grossedeepdrebin} under two representative drift scenarios: intra-family drift (Airpush\_tr $\rightarrow$ Airpush\_te) and inter-family drift (Airpush\_tr $\rightarrow$ Hiddad\_te, where Hiddad does not appear in training). These settings directly correspond to the malware evolution scenarios discussed in our Motivation (Section~\ref{sec:Malware Evolution}). 

These two families belong to adware and share a common logic: detecting user activity to trigger advertisements and verifying connectivity to deliver content. Our analysis reveals that \model\ achieves superior robustness by capturing the fundamental behavioral intent, which remains stable across families and versions. Specifically, \model\ successfully identifies these invariant features associated with the malware lifecycle and broad network capabilities. For instance, it consistently assigns high importance to system-wide broadcasts like \texttt{USER\_PRESENT} and \texttt{PACKAGE\_ADDED} (indicating when to activate) and coarse-grained checks like \texttt{ACCESS\_NETWORK\_STATE} (indicating capability). These signals abstract away from specific libraries, serving as stable indicators of malicious intent that persist even when the malware moves to a new family (Hiddad) or evolves over time. While the ERM-based DeepDrebin focuses heavily on lower-level implementation artifacts used to realize these behaviors in specific training samples (a consequence of the given feature space), it prioritizes concrete API calls (e.g., \texttt{getRunningTasks}) or narrowly scoped permissions (e.g., \texttt{SYSTEM\_ALERT\_WINDOW}) that are tightly coupled to specific Android versions or family-specific coding choices. Overall, this comparison demonstrates that the F1-score improvement of \model\ stems from its ability to learn invariance, i.e., focusing on why a behavior occurs, rather than overfitting to how it is implemented.

% Our analysis shows that \model\ consistently assigns higher importance to stable, high-level intent and capability features that are less sensitive to version- or family-specific implementation changes. Under intra-family drift, \model\ emphasizes system-wide broadcast events such as \texttt{USER\_PRESENT} and \texttt{PACKAGE\_ADDED}, which are commonly associated with application activation and background service triggering and remain stable across different variants of the same family. In contrast, DeepDrebin places greater weight on specific APIs and permissions that are more prone to temporal variation. This difference becomes more pronounced under inter-family drift. When evaluated on the unseen Hiddad family, \model\ assigns higher importance to general network-related capabilities (e.g., \texttt{ACCESS\_NETWORK\_STATE}) and high-level lifecycle management, whereas DeepDrebin relies on more restrictive, version-reliant features. As a result, the dominant signals used by \model\ exhibit better transferability across families.

% Overall, this case study provides an interpretable explanation of why \model\ achieves improved F1-score under temporal drift: by favoring more stable intent prerequisites over brittle implementation-specific details, the model reduces its sensitivity to natural distribution shifts induced by malware evolution.



\vspace{0.5em}
\noindent\textbf{Response R1.5 [Threat to Validity]} \textit{Please clarify the potential threats to the validity of your experiment in a dedicated section.}

We have added a dedicated Threat to Validity section (Section~\ref{sec:threat}) to discuss factors that may affect the interpretation of our results. In this section, we clarify potential threats to internal validity (e.g., model complexity and hyper-parameter sensitivity), construct validity (e.g., using temporal partitioning as an agnostic proxy for malware drift), and external validity (e.g., focusing on natural temporal drift rather than adversarial shifts). These discussions help delineate the scope of our conclusions and the assumptions underlying our evaluation.


\vspace{0.5em}
\noindent\textbf{Response R1.6 [Artifacts]} \textit{Did you provide the artifact for your work to allow open science?}

We have made our code publicly available at \texttt{https://github.com/ZhengXR930/IRM.git}. The repository also provides detailed descriptions of the datasets and experimental settings.


\vspace{1.5em}
{\large\noindent\textbf{Response to Reviewer 2}}

\vspace{0.5em}
\noindent\textbf{Response R2.1 [Detailed Comparisons \& Reasons behind Good Results]} \textit{The authors discussed different drift-robust malware detectors in the Background section. I would love to see more in-depth and detailed comparisons between TIF and these techniques especially the most similar ones (i.e., the first category). While the current discussions discussed the limitations of these techniques, it is not very clear how and why TIF can address these limitations. From a very high-level understanding, both TIF and some existing techniques focus on the invariant features across different time periods. It is unclear what novel design of TIF makes it outperform the existing techniques. In other words, I would like to suggest the authors to add more detailed introductions to the most similar techniques, connect their limitations with the challenges discussed in the motivating example if possible, and add intuitions on how TIF can address these limitations.}

We have substantially revised the manuscript to clarify both the conceptual differences between \model\ and the most related drift-robust techniques, and the reasons why \model\ achieves superior robustness under realistic malware evolution. 

From a theoretical perspective, existing static drift-robust methods address drift by attributing performance degradation to specific assumed causes or manifestations. As we discussed in Section~\ref{Drift-robust Malware Detectors}, APIGraph~\cite{apigraph} assumes drift is primarily driven by API raplacement and stabilizes the feature space accordingly; T-stability~\cite{svm_ce} and related training-dynamics-based methods~\cite{scrr} assume that unstable features can be identified through monotonic temporal trends or learning-speed heuristics; family-aware methods~\cite{DOMR} focus on the emergence of unseen families as the dominant source of drift. While effective under the particular scenarios they model, these approaches inherently rely on restrictive assumptions about how drift is reflected in the feature space. In practice, malware evolution is driven by multiple, interacting factors, and the same high-level behavior may persist even when APIs remain unchanged, but implementation strategies evolve. Under such conditions, assumptions tied to a single drift source may no longer hold and thus fail to generalize. In contrast, \model\ does not assume any specific cause of drift. Instead, it takes a manifestation-oriented perspective: if malware evolution induces distribution shifts over time, then time itself provides weak but consistent supervision for exposing unstable correlations. \model\ explicitly treats temporal partitions as environments and reformulates training to distinguish correlations that persist across time from those that vary with time, rather than predefining what should be stable. By breaking the ERM paradigm that collapses all temporal data into a single distribution, \model\ enables the learning process to surface and suppress temporally unstable shortcuts while preserving invariant semantics. This design choice fundamentally differentiates \model\ from prior approaches that either filter features based on assumed drift patterns or rely on post-hoc updates to compensate for drift.

Beyond this conceptual distinction, we have strengthened the empirical explanation through a case study (Section~\ref{sec:case study}). \model\ consistently emphasizes features aligned with malicious intent and behavioral prerequisites (e.g., lifecycle events, network capability, persistent background execution), rather than implementation-specific APIs or permissions that are brittle under evolution. In contrast, ERM-based and feature-constrained baselines increasingly rely on volatile, version-dependent signals. The case study provides concrete evidence that \model\'s training objective leads to representations that are both more stable and more semantically meaningful under temporal drift.

Taken together, the novelty of \model\ lies in changing the training paradigm itself: it leverages temporal structure to learn invariance without prespecifying drift causes and without relying on frequent retraining. This principled shift explains why \model\ consistently outperforms existing drift-robust methods across diverse drift scenarios.


\vspace{0.5em}
\noindent\textbf{Response R2.2 [Baseline Selection]} \textit{How are the baselines selected? There are different existing techniques that aim to address the problem of evolving malware families. How did the authors come to these 3.}

We thank the reviewer for this question. Our baseline selection follows a principled criterion: we compare against methods that address malware distribution drift under the same task definition and evaluation protocol, and whose robustness mechanisms align with the problem formulation discussed in our Introduction (Section~\ref{sec:introduction}) and Background (Section~\ref{Drift-robust Malware Detectors}). 

Both static and continual learning baselines are included. For the static ones, we focus on approaches that enhance detector robustness under a static, offline training setting, without relying on deployment-time updates or auxiliary supervision.
Within this scope, we select three representative baselines that correspond to complementary and widely adopted perspectives on handling malware drift. Rather than differing only by implementation details, these methods reflect distinct mainstream design philosophies:
(i) APIGraph~\cite{apigraph} represents approaches that explicitly assume the cause of drift, attributing performance degradation primarily to API-level implementation changes and addressing drift via feature selection;
(ii) T-stability~\cite{svm_ce} represents approaches that characterize drift through its observable temporal heuristics, constraining features whose discriminative power varies across time;
(iii) Guided Retraining~\cite{guide_retraining} represents a general, model- and feature-agnostic representation enhancement strategy that improves robustness without making explicit assumptions about drift sources. Together, these methods span a spectrum from explicit assumptions about drift causes, to empirical observations of drift effects to assumption-free representation enhancement. This categorization mirrors the landscape of existing solutions discussed in our Background section and enables a systematic comparison with our approach from multiple complementary angles.

In addition, we include HCC~\cite{continuous} as a continual learning-based baseline. Unlike the static methods above, HCC mitigates drift by periodically updating the model with newly observed samples during deployment. We include this baseline not as a direct competitor in the static setting, but to evaluate whether our framework can also serve as a robustness enhancement when integrated into a dynamic, deployment-time update pipeline, thereby assessing its effectiveness in both static and continual scenarios.

We do not include DOMR~\cite{DOMR} because it relies on episodic meta-learning with one-vs-rest recognition heads tailored for identifying new malware families, which is incompatible with our setting involving hundreds of families and both inter- and intra-family drift. SCRR~\cite{scrr} is excluded due to the unavailability of its source code and its highly sensitive bi-level optimization procedure, making faithful reproduction without an official implementation impractical.



\vspace{0.5em}
\noindent\textbf{Response R2.3 [Continual/Incremental Learning Comperison]} \textit{As far as I understand, the authors did not compare with incremental training techniques as baselines. The authors may include a representative technique as baseline or give good reasons on why they chose not to include such a baseline.}

We clarify that our evaluation explicitly includes a representative continual learning baseline and a dedicated research question to assess performance under incremental model updates.

Specifically, we include HCC~\cite{continuous}, a state-of-the-art continual learning framework for Android malware detection, as our representative baseline. HCC addresses distribution drift by periodically detecting drifted samples and updating the model during deployment, and is widely adopted in this domain. In the context of malware detection, incremental training is commonly realized as a form of continual learning, where models are periodically updated with newly observed samples to handle distribution drift. HCC follows this paradigm and therefore serves as a representative incremental/continual learning baseline.

Moreover, we design a dedicated research question (RQ4) (Section~\ref{sec:continual}) to systematically evaluate the interaction between \model\ and continual learning. In this evaluation, we consider two complementary settings based on HCC:
\textit{(i) Without the continual update mechanism}, where model updates are disabled to isolate and directly compare representation quality. Under this setting, \model\ achieves an average F1 improvement of 49.16\% on drift samples compared to HCC, indicating substantially more stable and discriminative representations.
\textit{(ii) With the continual learning framework enabled}, where we follow HCC’s update strategy to evaluate the full detection pipeline under realistic drift conditions. In this setting, \model\ reduces the number of required model updates from 65 to 38, cutting labeling cost by 41.5\% while maintaining comparable detection performance.


This separation allows us to disentangle improvements arising from stronger representations from those due to continual adaptation. Our results show that \model\ learns more stable representations that delay performance degradation, thereby reducing update frequency and labeling cost when integrated into a continual learning framework, while maintaining detection performance.



\vspace{0.5em}
\noindent\textbf{Response R2.4 [Precision \& Recall]} \textit{For the evaluation, the authors only presented F1-score and AUT. While I understand that F1-score is a combination of Precision and Recall. Can the authors still add the precision and recall values to provide a more comprehensive picture of the performance of TIF?}

We thank the reviewer for this suggestion. Malware detection is a highly imbalanced classification problem in both training and testing phases (malware: benign = 1:10), under which precision and recall are highly sensitive to class imbalance and threshold choice. Reporting either metric in isolation can therefore be misleading, especially under temporal drift, where score distributions shift over time. We adopt F1-score as the primary metric because it provides a balanced summary of precision and recall that is more robust to class imbalance. Based on this consideration, AUT(F1)~\cite{tesseract}, a widely used metric, is further used to characterize long-term performance stability, which would be less meaningful if applied to precision or recall alone due to their high variance in this setting. In addition, to demonstrate that our results reflect consistent trends rather than single-run variability, we have additionally reported the standard deviation across multiple runs in Table~\ref{tab:rq1}. The low variance observed across runs indicates that the performance gains of \model\ are stable and reproducible, providing further evidence of its effectiveness beyond point estimates of evaluation metrics. 


\vspace{0.5em}
\noindent\textbf{Response R2.5 [Performance Trend of T-stability]} \textit{In table 1, interestingly, for Drebin with T-stability, the increases are higher in later years. The gaps between the improvement of T-stability and TIF is narrowing. Could the authors add some explanations on why this happened?} 

We thank the reviewer for this insightful observation.
The narrowing gap can be attributed to how different methods handle the trade-off between discriminability and temporal stability. In the early stages, TIF holds a clear advantage because it jointly optimizes for stability and discriminability in the representation space, allowing it to preserve features that are both predictive and consistent across time. In contrast, T-stability applies conservative, feature-level constraints that suppress temporally unstable features, even when they are highly discriminative in the early phase, leading to lower initial performance.

As time progresses, features that lack temporal robustness naturally lose their predictive value under time-aware evaluation. Since both T-stability and TIF emphasize temporally stable patterns, the effective feature sets used by the two methods become more similar over time, which explains the observed narrowing of the performance gap.

Despite this convergence, TIF consistently outperforms T-stability. T-stability operates purely at the feature level with linear constraints and follows a suppressive strategy, limiting its ability to model complex feature interactions. In contrast, TIF performs invariant learning in a non-linear representation space and explicitly optimizes both stability and discriminability, enabling it to retain more expressive and robust semantics throughout the evaluation period.

We note that our case study (Section~\ref{sec:case study}) analyzes feature importance in the Drebin space purely for interpretability. The observed feature-level behaviors are manifestations of the underlying representation learned by TIF, which is optimized in the representation space rather than through explicit feature-level constraints.


\vspace{0.5em}
\noindent\textbf{Response R2.6 [Explanation of Results in RQ2]} \textit{The evaluation setup is a bit confusing for RQ2. How are the values calculated in Figure 6? I’m not very sure about this. This makes it hard to interpret the results. Would the authors add some explanations on the experiment set up for this RQ?}

We have revised the manuscript to clarify both the experimental design and the calculation of Figure~\ref{fig:rq2}, making the evaluation procedure more explicit. First, we clarify the design motivation of RQ2, which is to examine whether the proposed framework can learn invariant representations under both intra-family and inter-family drift, corresponding to the two types of temporal invariance discussed in Section~\ref{sec:Malware Evolution}. To this end, we explicitly define two evaluation settings in Section~\ref{Dataset}: 1) Closed-world, where test samples contain only malware families observed during training to evaluate intra-family invariance; and 2) Open-world, where test samples contain only malware families absent from the training set to evaluate inter-family invariance. To ensure fair comparison under highly imbalanced family distributions, test samples in each setting are sorted chronologically and partitioned into 10 equal-sized temporal segments, which are used consistently across RQ2. 

Second, we recreated Figure~\ref{fig:rq2} to make it cleaner, measuring representation stability. For each temporal test segment, we extract the hidden representations of malware samples from the encoder and compute their mean embedding. We then compute the cosine similarity between this mean test embedding and the mean malware embedding of the training set. This procedure is applied consistently under both closed-world and open-world settings. The results in Figure~\ref{fig:rq2} therefore quantify how closely the representations learned at test time remain aligned with those learned during training. Higher similarity indicates more stable representations under temporal distribution drift. We have incorporated these explanations into Section~\ref{rq2} to improve clarity and interpretability.


\vspace{0.5em}
\noindent\textbf{Response R2.7 [RQ3 and Corresponding Figures]} \textit{The formatting for RQ3 and the figures may be revised. }

We have revised the presentation of RQ3 to improve clarity and interpretability. First, we clarify the evaluation protocol by defining the closed-world and open-world settings in the Dataset section (Section~\ref{Dataset}) and explaining that the indices in Table~\ref{tab:rq3} correspond to successive temporal test segments with equal sample sizes. Second, we refine the explanation of the Feature Contribution Score (FCS). We clarify that FCS measures the extent to which a model assigns importance to features that are discriminative in the current evaluation set, and that temporal invariance is inferred from the persistence of high FCS values across successive time segments rather than from the absolute value at a single time point. These revisions align the definition of FCS, the experimental protocol, and the presentation of Table~\ref{tab:rq3}, thereby improving the clarity of RQ3.


\vspace{0.5em}
\noindent\textbf{Response R2.8 [Application Statistic]} \textit{The authors may also add the number of apps for each month or each year when conducting an evaluation regarding the changes over time.}

To provide a clearer picture of dataset evolution over time, we add a new table (Table~\ref{Dataset}) that summarizes, for every evaluation year, the numbers of benign and malicious samples, as well as the number of seen and unseen malware families appearing in the test set to make the temporal dynamics of the dataset explicit.


\vspace{1.5em}
{\large\noindent\textbf{Response to Reviewer 3}}


\vspace{0.5em}
\noindent\textbf{Response R3.1 [Baseline Selection]} \textit{It is unclear why the authors selected the three techniques as representatives. Why did the authors not select the latest technique of each kind? I would like to see more explanations} 

We thank the reviewer for this comment. Our baseline selection is guided by alignment with our problem setting and by representativeness of the mainstream robustness paradigms discussed in the Introduction (Section~\ref{sec:introduction}) and Background (Section~\ref{Drift-robust Malware Detectors}), rather than by recency alone. As clarified in Response R2.2, our goal is to compare against methods that explicitly target robustness to evolving malware distributions \emph{under the same static, offline training setting}, without relying on deployment-time updates or auxiliary supervision. 

All selected baselines operate under the same static, offline training setting as our method, making them directly comparable. More importantly, they represent complementary and widely adopted perspectives on handling malware drift, more detailed information is also discussed in Response R2.2:
(i) APIGraph~\cite{apigraph} represents approaches that explicitly assume the cause of drift (e.g., API-level changes);
(ii) T-stability~\cite{svm_ce} represents approaches that characterize drift through its observable temporal behavior of features;
(iii) Guided Retraining~\cite{guide_retraining} represents a general model and feature agnostic representation enhancement strategy that does not rely on any explicit assumption about drift causes.

In addition, we include a continual learning baseline, HCC~\cite{continuous}, to evaluate whether our framework can also serve as a robustness enhancement when combined with deployment-time model updates. Together, these baselines are consistent with the categories of existing solutions outlined in our Introduction and Background, and enable a multi-angle evaluation of effectiveness across different mainstream design philosophies. Moreover, these methods represent the most recent reproducible works that satisfy the comparison criteria of \model.


\noindent\textbf{Response R3.2 [Dataset Information]} \textit{The authors may also add the number of apps for each month or each year when conducting an evaluation regarding the changes over time.} 

Following this comment, we augment the dataset description with detailed temporal statistics. In particular, we include Table~\ref{tab: dataset} that reports the yearly number of benign and malicious applications used in our evaluation, together with the number of visible (seen during training) and previously unseen malware families in each test year. This revision provides a transparent and fine-grained view of how the dataset evolves over time and how the evaluation settings relate to realistic deployment scenarios under temporal drift.


\vspace{0.5em}
\noindent\textbf{Response R3.3 [Latest Malware]} \textit{In the experiments, the malware samples are all before 2023. The latest malware samples in 2024 and 2025 are not included for experiments. I would suggest that the authors extend their experiments to include the latest samples.}

In response, we have extended our dataset to include malware samples collected up to June 2025. We note that, after mid-2025, the number of newly available malicious samples on AndroZoo becomes extremely limited (on average fewer than 15 malicious samples per month), which is insufficient to form a representative evaluation set and may introduce statistical bias. Therefore, we include all available samples up to June 2025 and clearly justify this cutoff in the revised manuscript. Accordingly, we update Table~\ref{tab:rq1}, extend the experimental results to cover these newer samples, and revise the dataset description (Section~\ref{Dataset}) to explain the data selection and filtering process explicitly. These changes ensure that our evaluation reflects the most recent malware evolution while maintaining statistical reliability.


\vspace{0.5em}
\noindent\textbf{Response R3.4 [Statistical Analysis]} \textit{The experiments were repeated only three times (Section V), which is a relatively limited for evaluating model stability. Moreover, the lack of statistical analysis (e.g., variance, confidence intervals, or significance testing) reduces confidence in the reported improvements. Including such analyses would strengthen the experimental results.}

Following the suggestion, we further strengthen the analysis by explicitly reporting variability. Specifically, we add the standard deviation across three random seeds for \model\ in the main result table (Table~\ref{tab:rq1}). The results show consistently low variance across different runs, demonstrating that the observed performance gains are stable and reproducible rather than artifacts of a particular initialization. 



\vspace{0.5em}
\noindent\textbf{Response R3.5 [Interpretation of Experimental Results]} \textit{Some experimental results lack sufficient interpretation. For example, in Table V, the best performance for years 2020–2022 is achieved by the MPC1+IGA combination, yet this finding is not discussed in depth. Similarly, in Table VI, the best performance for years 2019–2023 does not correspond to monthly segmentation, which appears to contradict the interpretation in Section V-F. Providing more detailed explanations for these inconsistencies would improve the clarity and credibility of the empirical analysis. Besides, the current analyses are mostly based on metric values. I would suggest that the authors perform a deeper analysis to find out some temporal invariants TIF learned when combined with each kind of detector for discussion.}

We revised explanations on these Tables and the corresponding results:

\textbf{Interpretation of Table~\ref{tab: ablation}}: Since our samples are collected from real-world Android platforms, the dataset naturally reflects the evolution of malware development techniques. In recent years, Android malware and many high-risk apps increasingly employ commercial packing and aggressive obfuscation/anti-analysis techniques, which have become a major obstacle for static and dynamic security analysis~\cite{xue2021happer}. Such samples weaken the reliability and consistency of static feature signals, making discriminative patterns noisier and less aligned with those observed during training~\cite{aghakhani2020malware}. As a result, the cross-environment consistency signal required for invariant learning becomes harder to estimate.

Under this regime, stronger invariance-inducing regularization introduced by MPC2 may over-constrain the representation space and suppress residual discriminative structures that remain useful, leading to diminished or unstable gains. In contrast, MPC1 combined with IGA provides a more moderate regularization strength: MPC1 encourages partial sharing across environments without forcing strict alignment, while IGA suppresses environment-specific shortcuts. This balance makes MPC1+IGA more effective during the 2020–2022 period, where discriminative signals still exist but are increasingly noisy. The marginal increase observed in 2023 (from 0.662 to 0.665) is small and falls within expected year-to-year fluctuations. It does not indicate a systematic recovery of strong alignment benefits, but rather reflects the heightened sensitivity of heavily regularized models to year-specific drift characteristics under long-term evolution. Importantly, this observation does not imply a fundamental limitation of \model. As discussed in Section~\ref{sec:continual}, we further demonstrate that \model\ can be integrated into a continual learning framework to enable knowledge updating and progressively improved representations under evolving distributions although there are packed or obfuscated samples.

\textbf{Interpretation of Table~\ref{tab: env}}: The apparent inconsistency between the monthly result and quarterly result arises from the interaction between environment granularity and the temporal scale of distribution drift. Monthly segmentation provides finer-grained environments and is effective when distribution shifts are relatively mild, particularly in earlier test periods. In such cases, frequent temporal partitions help expose subtle variations and enable the model to learn invariances that are robust to short-term evolution. This explains why monthly segmentation can achieve strong performance in early stages. However, monthly partitions induce only small distributional contrasts, which may be insufficient to expose unstable correlations that emerge over longer time horizons. In contrast, quarterly segmentation introduces stronger temporal contrasts while maintaining sufficient samples per environment, enabling the model to better capture invariances that generalize across larger temporal gaps. Therefore, the superior performance of quarterly segmentation in later years reflects a trade-off between granularity and representativeness, and is consistent with the role of environment design discussed in Section~\ref{env seg}, and we have revised this section for clearer illustration.

In addition, we have added a case study (Section~\ref{sec:case study}) to provide a qualitative analysis of the temporal invariants learned by \model\ beyond metric-based evaluation. Using the interpretable Drebin~\cite{Arpdrebin} feature space and attribution analysis, we examine how \model\ reshapes feature importance under both intra-family and inter-family temporal drift. The case study shows that \model\ consistently emphasizes intent-level features that are intrinsic to malicious behavior and remain stable across time and families, while suppressing implementation-specific APIs and permissions that are brittle under evolution. These observations offer concrete evidence that \model\ learns semantically meaningful temporal invariants rather than relying on transient implementation shortcuts, explaining its superior robustness under temporal drift.

\vspace{0.5em}
\noindent\textbf{Response R3.6 [Deeper Analysis on Temporal Invariants Learned by \model]} \textit{Give a deeper analysis to find out some temporal invariants TIF learned when combined with each kind of detector for discussion.}

We have addressed it by adding a dedicated Case Study section (Section~\ref{sec:case study}) that provides a detailed interpretable analysis of the temporal invariants learned by \model. Case study focuses on two adware families aligning with motivation section (Section~\ref{motivation}). By examining the feature importance changes under drift, we found that \model\ learns to rely on relatively invariant features related to malware behavior, rather than transient implementation shortcuts. Specifically, the analysis shows that \model\ extracts temporal invariants at two levels: activation logic and capability requirements. It consistently emphasizes stable lifecycle triggers (e.g., \texttt{USER\_PRESENT} for device unlocking) and essential network permissions, which represent the core operational logic of adware that persists over time. Conversely, the baseline model (ERM-based model) overfits to volatile API usages that shift with Android updates. This analysis confirms that the ``temporal invariants'' learned by our framework are meaningful abstractions of malicious intent, explaining why \model\ can maintain effectiveness across different time periods and malware families.

% In this case study, we analyze feature attributions in the interpretable Drebin feature space and examine how \model\ reshapes feature importance under both intra-family and inter-family temporal drift, in comparison with an ERM-based detector. The analysis reveals that, when combined with standard malware detectors, \model\ consistently emphasizes stable, intent- and capability-level features that persist across time and families, while suppressing volatile, implementation-specific APIs. This analysis provides concrete evidence that \model\ learns semantically meaningful temporal invariants rather than relying on transient shortcuts, thereby explaining its superior robustness under temporal distribution drift.

\vspace{0.5em}
\noindent\textbf{Response R3.6 [Overhead]} \textit{What is the overhead of the approach?} 

We have clarified the overhead of the proposed approach in Section~\ref{sec:overhead}. From the inference perspective, \model\ introduces zero inference-time overhead. All auxiliary modules (e.g., environment partitioning, contrastive heads) are used solely during optimization. The deployed model shares the same architecture and latency as the baseline. From the training perspective, while \model\ incurs a predictable increase in offline training computation, this is a strategic investment to ensure robustness. By learning drift-invariant representations, \model\ maintains performance stability longer than ERM. This significantly reduces the frequency of necessary model updates (retraining and labeling) in continual learning scenarios, thereby lowering the total operational cost over the model's lifecycle.

% We have clarified the overhead of the proposed approach in Section~\ref{sec: overhead}. Specifically, we present a detailed per-iteration complexity analysis of both training stages and show that the overall cost is dominated by the standard ERM encoder training, with the additional components contributing only a small constant-factor overhead. This conclusion follows from the fact that the introduced operations scale linearly with batch size and representation dimension, while the encoder forward/backward cost scales quadratically. Consequently, the proposed framework does not introduce asymptotic overhead, does not grow with deployment time, and incurs no inference-time cost. In addition, we utilize \model\ in the continual learning setting, the result shows that purposed model decrease update cost by 41.5\%.
